Concise Answers to Complex Questions: Summarization of Long-form Answers

Long-form question answering systems provide rich information by presenting paragraph-level answers, often containing optional background or auxiliary information. While such comprehensive answers are helpful, not all information is required to answer the question (e.g. users with domain knowledge do not need an explanation of background). Can we provide a concise version of the answer by summarizing it, while still addressing the question? We conduct a user study on summarized answers generated from state-of-the-art models and our newly proposed extract-and-decontextualize approach. We find a large proportion of long-form answers (over 90%) in the ELI5 domain can be adequately summarized by at least one system, while complex and implicit answers are challenging to compress. We observe that decontextualization improves the quality of the extractive summary, exemplifying its potential in the summarization task. To promote future work, we provide an extractive summarization dataset covering 1K long-form answers and our user study annotations. Together, we present the first study on summarizing long-form answers, taking a step forward for QA agents that can provide answers at multiple granularities.

==> figs/fig_1.tex <==
\begin{figure}
    \small
    \centering
    \begin{tabular}{|p{208pt} |}
        \hline \\
        \textbf{Q:} What is the social construction of reality in sociology? \vspace{0.2em} \\
        \textbf{Original Answer:} Berger and Luckmann introduced the term "social construction" into the social sciences and were strongly influenced by the work of Alfred Schütz. \hlc[lightred]{-Their} \hlc[lightblue]{+Berger and Luckmann's} \hlc[lightgreen]{central concept is that people and groups interacting in a social system create, over time, concepts or mental representations of each other's actions, and that these concepts eventually become habituated into reciprocal roles played by the actors in relation to each other.} When these roles are made available to other members of society to enter into and play out, the reciprocal interactions are said to be institutionalized.  In the process, meaning is embedded in society. \hlc[lightgreen]{Knowledge and people's conceptions (and beliefs) of what reality is become embedded in the institutional fabric of society. Reality is therefore said to be socially constructed.} \vspace{0.5em} \\
        \textbf{Abstractive Summary:} Social construction of reality was introduced into the social sciences by Berger and Luckmann. Their central concept is that people and groups interacting in a social system create, over time, concepts or mental representations of each other's actions. \vspace{0.5em} \\
        % \textbf{Decontextualized Extractive Summary:}   central concept is that people and groups interacting in a social system create, over time, concepts or mental representations of each other's actions, and that these concepts eventually become habituated into reciprocal roles played by the actors in relation to each other.
        %  \\
         \hline 
    \end{tabular}
    \caption{An example question, long-form answer pair and its summaries. We show the extractive gold summary (highlighted in green) with an automatic decontexutalization edit (\hlc[lightred]{-Their} \hlc[lightblue]{+Berger and Luckmann's}). The summary from an abstractive model~\cite{pegasus} is shown below.}
    \label{fig:sampleSummary}
\end{figure}
